Dynamic Solutions for Hybrid Quantum-HPC Resource Allocation

The integration of quantum computers within classical High-Performance Computing (HPC) infrastructures is receiving increasing attention, with the former expected to serve as accelerators for specific computational tasks. However, combining HPC and quantum computers presents significant technical challenges, including resource allocation. This paper presents a novel malleability-based approach, alongside a workflow-based strategy, to optimize resource utilization in hybrid HPC-quantum workloads. With both these approaches, we can release classical resources when computations are offloaded to the quantum computer and reallocate them once quantum processing is complete. Our experiments with a hybrid HPC-quantum use case show the benefits of dynamic allocation, highlighting the potential of those solutions.

==> OLD-PARTS.tex <==
\section{State-of-the-art}\label{sec:background}

HPC-QC integration is undoubtedly a hot topic being actively investigated at research level~\cite{schulzAcceleratingHPCQuantum2022a,humbleQuantumComputersHighPerformance2021,bartschvaleriaQCHPCQuantum2021,brittHighPerformanceComputingQuantum2017,mccaskeyXACCSystemlevelSoftware2020}, promoted by quantum computing vendors~\cite{ruefenachtBringingQuantumAcceleration}, and being funded by prominent initiatives like EuroHPC and the Quantum Flagship framework\footnote{\url{https://doi.org/10.3030/101018180}}~\cite{binosiEuroQCSEuropeanQuantum}. These efforts significantly contribute to the classification of quantum applications~\cite{humbleQuantumComputersHighPerformance2021}, the definition of HPC-QC architectures~\cite{bartschvaleriaQCHPCQuantum2021,humbleQuantumComputersHighPerformance2021,beck2024quantum}, and the definition of a shared software stack~\cite{humbleQuantumComputersHighPerformance2021,schulzAcceleratingHPCQuantum2022a,willeMQT}. On the other hand, the discussion about programming models is limited~\cite{mccaskeyXACCSystemlevelSoftware2020, schulzAcceleratingHPCQuantum2022a} and mainly assumes digital architectures.
%Current quantum computers can be considered on-demand, large-scale, standalone experimental racks: sometimes they need cryogenics, sometimes optical benches, and, most of the time, they are susceptible to the installation environment (e.g., EM fields, temperature, humidity, and vibrations). 
However, the field characteristics different computational models (i.e., digital and analogue~\cite{henrietQuantumComputingNeutral2020}) and different hardware technologies, all with their peculiar characteristics and requirements. One of the consequences is that quantum machines are typically installed in lab-like environments, far from operational data centres, and accessed via a public network through high-level languages and dedicated libraries~\cite{Qiskit,pulser}. Through these tools, users can define kernels (i.e., circuits), send them to the machine via Representational State Transfer (REST) Application Programming Interfaces (APIs) and solve them in a sequential, mostly single-threaded fashion.

While the cloud access model is fine for the possibilities of current quantum machines, it is far from a proper HPC integration, which should leverage direct connection through a high bandwidth medium and higher control of the underlying quantum hardware. Despite some effort to set up dedicated connections\footnote{\url{https://www.vttresearch.com/en/news-and-ideas/finland-opens-quantum-computer-research-purposes-fusion-quantum-computing-and}} and data centre co-locations\footnote{\url{https://eurohpc-ju.europa.eu/selection-six-sites-host-first-european-quantum-computers-2022-10-04\_en}}, current approaches to HPC-QC still heavily rely on the same access model as cloud services. Moreover, there is not a single view on how the proper HPC-QC integration should happen, as the technology is still too young. Nonetheless, we can classify the HPC-QC integration types into three categories, following the solutions suggested in the literature: 

\begin{itemize}
    \item \emph{Tightly coupled}: classical computation happens within the coherence time of the quantum machine%(c.f. \emph{in-sequence-processing}~\cite{humbleQuantumComputersHighPerformance2021})
    , and affects the execution of the circuit. The main use case for this is error correction (i.e., by mid-circuit measurements and syndrome extraction), which \emph{we do not consider being HPC-QC}, but an exclusive matter of quantum hardware. On the other hand, it is possible to envision a future where a classical process (e.g., an MPI rank) interacts with a running quantum circuit to achieve something more than error correction, but this goes well beyond the scope of the near-future integration scenarios. 
    \item \emph{Quantum offloading}: the typical circuit execution used to accelerate specific operation (i.e., quantum kernels). It can be either synchronous or asynchronous, but the classical code is in charge of the control flow and keeps running until the end.
    \item \emph{Loosely-coupled} (workflows): an external workflow manager (it can be as simple as a shell script) is in charge of the control flow. Classical and quantum resources are allocated separately for each step once that step is ready to run.
\end{itemize}
The first mode still requires a significant advancement in hardware maturity, hence it will not be discussed in the scope of this paper, which focuses on the use-cases for the second and third integration modes.




\section{Current HPC-QC integration challenges}\label{sec:challenges}
%The workloads discussed in Section \ref{sec:taxonomy} highlight how 
Any practical integration solution must support interleaved and overlapped HPC and quantum tasks, along with concurrent, multi-tenant access to quantum resources. In this context, we identified three specific challenges we need to address.

\noindent\textbf{Software heterogeneity. }
The software used by QC applications differs substantially from the one classically employed in the HPC field: while the first relies heavily on interpreted languages (e.g., Python or Julia), the second uses mainly compiled performance-oriented languages like C/C++/Fortran and libraries like MPI, OpenMP and CUDA. While some efforts have already addressed this difference, providing tools to bridge this disparity~\cite{mccaskeyXACCSystemlevelSoftware2020,gazdaPragmaBasedFramework2024,schulzAcceleratingHPCQuantum2022a}, there is not a de-facto standard for HPC-QC hybrid programming. This lack of a single shared programming layer makes reasoning about a generic HPC-QC application difficult, and the quantum machines' heterogeneity only worsens the matter. In general, as we move the QC field towards the HPC one, we should opt out of interpreted languages, as their strengths (faster prototyping) get outweighed by the possible improvements in performance obtained through HPC languages and libraries. 



\noindent\textbf{Access and allocation model. }
%As discussed in Section~\ref{sec:sota}, 
Current quantum computers typically provide access through dedicated libraries and REST APIs, with an internal queue that allows for asynchronous job submission and multi-user operation. Access to this API is regulated through dedicated accounting systems and, in principle, anyone with existing access to the API can submit jobs anytime. This does not play well with operational HPC, where access to resources is regulated by job schedulers based on specific policies. Moreover, each vendor currently provides its own dedicated API, that requires dedicated solutions.

\begin{figure}[t]
  \centering
  \includegraphics[width=0.8\linewidth]{Fig/timescale.png}
  \caption{Time scales of relevant quantum jobs/shots. The job on neutral atoms machine includes the calibration time for an arbitrary register geometry.}\label{fig:timescale}
\end{figure}

Given this situation, the first critical challenge is the integration of the QPU vendor mechanisms into a scenario based on batch schedulers and well-established accounting systems: we need some mechanism to integrate QPUs provided as web services into the picture of the operational HPC accounting and scheduling system, respecting the policies set by, e.g., SLURM~\cite{slurm}.

\noindent\textbf{Workload imbalance. }
Beyond the access model, it is necessary to understand that the characteristic time scales of quantum jobs can heavily affect the job scheduling. In fact, while the time taken by classical computation strongly depends on the specific algorithm and the size of the input data, the time taken by a quantum kernel execution is largely driven by the specific QPU technology and, to a lesser extent, by the amount of statistics to be collected (i.e., shots). In particular, depending on the technology chosen, the time taken by a quantum job could vary significantly (see Figure~\ref{fig:timescale}) and we can envision scenarios where typical HPC batch schedulers fall short in terms of efficient use of resources due to workload imbalance.

To clarify this point, we can use as an example the job in Listing~\ref{lst:hetjob}, describing a job \emph{co-scheduling} 10 nodes in a classical partition and 1 QPU (defined as a SLURM gres, more on that in Section~\ref{sec:approach}) in a quantum partition, both for 1 hour.
\begin{lstlisting}[basicstyle=\ttfamily\footnotesize,float,floatplacement=t,language=Bash, caption=Example of SLURM job script to run a potential HPC-QC hybrid job, label=lst:hetjob]
#!/bin/bash
#SBATCH --partition classical
#SBATCH --nodes 10
#SBATCH --time=01:00:00

#SBATCH hetjob

#SBATCH --partition quantum
#SBATCH --gres=qpu:1
#SBATCH --time=01:00:00

srun ./hybrid_job
\end{lstlisting}
Let us consider a superconducting QPU for which we can assume that each quantum task will last $<10 \, \textrm{s}$ (see Figure~\ref{fig:timescale}): even with many tasks launched inside the job, this can lead to a heavy under-utilisation of the QPU that is exclusively allocated to this job for one hour. Conversely, if the QPU is based on neutral atoms, a quantum task could easily last more than $30 \, \textrm{min}$, leading to under-utilisation of the classical nodes that will be idle waiting for the quantum job completion. These issues must be taken into account when integrating quantum hardware within HPC facilities to ensure efficient resource allocation: plain co-scheduling of resources with exclusive access to QPUs is not sufficient.
